Opinion Dynamics with Set-Based Confidence: Convergence Criteria and Periodic Solutions

This paper introduces a new multidimensional extension of the Hegselmann-Krause (HK) opinion dynamics model, where opinion proximity is not determined by a norm or metric. Instead, each agent trusts opinions within the Minkowski sum $\xi+\mathcal{O}$, where $\xi$ is the agent's current opinion and $\mathcal{O}$ is the confidence set defining acceptable deviations. During each iteration, agents update their opinions by simultaneously averaging the trusted opinions. Unlike traditional HK systems, where $\mathcal{O}$ is a ball in some norm, our model allows the confidence set to be non-convex and even unbounded. We demonstrate that the new model, referred to as SCOD (Set-based Confidence Opinion Dynamics), can exhibit properties absent in the conventional HK model. Some solutions may converge to non-equilibrium points in the state space, while others oscillate periodically. These ``pathologies'' disappear if the set $\mathcal{O}$ is symmetric and contains zero in its interior: similar to the usual HK model, SCOD then converges in a finite number of iterations to one of the equilibrium points. The latter property is also preserved if one agent is "stubborn" and resists changing their opinion, yet still influences the others; however, two stubborn agents can lead to oscillations.

==> old_material.tex <==
%THIS IS A FILE FOR OLD TEXT, WHICH REMAINS OUTSIDE THE JOURNAL VERSION. WILL BE CLEANED and PUBLISHED on ArXiV later

%Part of Section II

\section{OLD MATERIAL}

\subsubsection{\bf Convergence of $n=2$ opinions}

We first notice that the GHK model with two agents always converges to an equilibrium, similar to usual BCOD models~\cite{Bernardo2024survey}.
\begin{lemma}\label{lem.n_2}
The opinions of $n = 2$ agents converge to finite limits, and the terminal opinion matrix  $\Xi(\infty)\dfb\lim_{t\to\infty}\Xi(t)$ is the equilibrium of system~\eqref{eq.HK}.
Additionally:
%\begin{enumerate}[(i)]

(i) If $\mathcal{O}$ is star-shaped at $\mathbf{0}$, the opinions either remain static $\Xi(t)\equiv\Xi(0)$
or reach consensus $\xi^1(\infty)=\xi^2(\infty)$;

(ii) If $\mathbf{0}$ is an internal point $\mathcal{O}$, the dynamics terminate at a finite number of steps:
$\Xi(t)=\Xi(\infty)$ for large $t$. \endofthm
%\end{enumerate}
\end{lemma}

\subsubsection{\bf A 3-periodic solution for $n=3$ scalar opinions}

In the case of scalar opinions ($d=1$), the confidence set is typically considered to be an interval (possibly, asymmetric) $\mathcal{O}=(-\ell,u)$, where $-\ell<0<u$. It is known that the opinion dynamics in this case terminate in a known number of iterations (polynomially depending on $n$)~\cite{2015_acc_coulson,2022_ECC_Bernardo,Bernardo2024survey}. Recent works~\cite{2020_vasca,bernardo2021heterogeneous}, focused on achieving of practical consensus in presence of homophily and heterophily effects, introduce a ``deadzone'' by considering the set $\mathcal{O}=(-\ell,-\varepsilon)\cup\{0\}\cup(\varepsilon,u)$.
We now show that, allowing $\mathcal{O}\subset\mathbb{R}$ to be a union of multiple intervals, it is possible to construct the GHK with $n=3$ agents that admits a \emph{periodic} trajectory.


%We accompany this example with several important remarks.

It is interesting to compare this example with the celebrated Sharkovsky theorem~\cite{BurnsHasselblatt2011_Sharkovsky}: If a \emph{continuous} discrete-time dynamical system on an interval has a fixed point of (minimal) period 3, it also has fixed points of all possible (minimal) periods. This theorem, evidently, does not apply to the GHK model, whose right-hand side is discontinuous. Furthermore, the system from Example~\ref{ex.period_1d_n3} and any GHK model with $n=3$ agents admits no solution of period 2.
\begin{lemma}\label{lem.n_3_no_period2}
Suppose that system~\eqref{eq.HK} with $n=3$ agents and some $\mathcal{O}\subseteq\mathbb{R}^d$ has a $T$-periodic solution $\Xi(t+T)\equiv\Xi(t)$. 
Then, first, either $T\geq 3$ or $\Xi$ is an equilibrium: $\Xi(t)\equiv\Xi(0)$. Second, the orbit $\{\Xi(t)\}$ is \emph{unidimensional}, i.e., points $\xi^1(t),\xi^2(t),\xi^3(t)$ all lie on a common line $\mathcal{L}$ (a 1-dimensional affine submanifold) in $\mathbb{R}^d$ for all $t$.\endofthm
\end{lemma}

\begin{remark}
The 3-periodic trajectory from Example~1, obviously, persists if set~\eqref{eq.setO-ex1} is shrunk to
\[
\mathcal{O}=(-1+\varepsilon,1-\varepsilon)\setminus\left(\mathcal{M}+(-\varepsilon,\varepsilon)\right),
\]
where $\varepsilon$ is small enough (reducing the maximal confidence range and removing each point from $\mathcal{M}$ with a small interval around it). 
This choice of $\mathcal{O}$ ensures that the periodic solution (locally) Lyapunov stable. Consequently, the set of initial conditions $\Xi(0)$ corresponding to diverging (non-convergent) solutions
has positive Lebesgue measure.
\end{remark}

\subsubsection{\bf Periodicity with a star-shaped confidence set $\mathcal{O}$}

One could argue that the key reason for the periodic oscillations in the previous example is the disconnected confidence set $\mathcal{O}$ (in fact, $\mathbb{R}$ admits no connected subsets except for intervals), caused by the ``punctured'' points. The next example demonstrates that, when dealing with multidimensional opinions, periodic solutions are possible even with a \emph{star-shaped}\footnote{Obviously, such a set is connected (and even path-connected) in $\mathbb{R}^d$.} confidence set.
Notice that if $\mathcal{O}$ is star-shaped at $\mathbf{0}$, then the following natural property holds: If an agent with opinion vector $\xi$ trusts another opinion $\xi'$, they trust all ``intermediate'' opinions falling in the interval $[\xi,\xi']$. 
Furthermore, choosing $n=4$, it is possible to get a solution of period $2$, which fails to exist in the case of $n=3$ agents.

%The next example demonstrates that even if the confidence set is star-shaped at $\mathbf{0}$, this is no longer enough to guarantee the convergence of two-dimensional opinions.
%\vspace{0.2cm}

\begin{comment}
\vspace{0.2cm}
\begin{example}\label{ex.period_1d}
Consider the confidence set $\mathcal{O} = \{(-3, 4) \setminus \mathbb{Z}\} \cup \{-3, 0, 4\}$. Choose the initial opinions of four agents have the values indicated in Fig.~\ref{fig.homo_period}.
Agents $2,3$ and $4$ will maintain their opinions unchanged over time, while the opinion of agent $1$ will alternate between $0$ and $2$ at even and odd time instants, respectively.
\begin{figure}[h!]
\center
  \includegraphics[width=6.5cm]{homo_period.jpg}
  \caption{Opinion $\xi^1(t)$ switches periodically between values $0$ and $2$.}
  \label{fig.homo_period}
\end{figure}
\end{example}
\end{comment}

\section*{Proof of Lemma~\ref{lem.n_2}}

%\begin{proof}
Denote $\eta(t)\dfb\xi^1(t)-\xi^2(t)\in\mathbb{R}^d$. In view of the BCOD~\eqref{eq.HK}, this variable evolves as follows
\[
\eta(t+1)=\mathfrak{P}(\eta(t))\eta(t),\;\;
\mathfrak{P}(\eta)\dfb
\begin{cases}
1, & \{\pm\eta\}\cap\mathcal{O}=\varnothing,\\
0, & \{\pm\eta\}\subseteq\mathcal{O},\\
\tfrac{1}{2}, &\text{otherwise}.\\
\end{cases}
\]
If $\mathfrak{P}(\eta(t_0))=1$, then the agents don't trust each other at iteration $t_0$, and the dynamics of BCOD terminate at equilibrium $\Xi(t_0)$.
If this does not happen, then $0\leq\mathfrak{P}(\eta(t))\leq 2^{-t}\,\forall t$. In view of~\eqref{eq.HK},
$\xi^1(t+1)-\xi^1(t)=-w_{12}(t)\eta(t)$ is an $\ell_1$-summable sequence, one shows the existence of $\xi^1(\infty)=\lim_{t\to\infty}\xi^1(t)$;
similarly, the limit $\xi^2(\infty)=\lim_{t\to\infty}\xi^2(t)$ exists, and $\xi^1(\infty)=\xi^2(\infty)$. The first part of Lemma is proven.
The statement (ii) is also obvious: assume that the BCOD does not terminate at an equilibrium. Then,
$\eta(t)\to 0$ as $t\to\infty$, and hence at some step $t_*$ one has $\eta(t_*)\in\mathcal{O}\cap\mathcal{-\mathcal{O}}$.
This leads to the contradiction: the dynamics do terminate at a consensus equilibrium at stage $t_*+1$, and
\[
\xi^1(t_*+1)=\xi^2(t_*+1)=\frac{1}{2}\left(\xi^1(t_*)+\xi^2(t_*)\right).
\]

To prove (i), notice that $\eta_0\in\mathcal{O}$ entails that $\varepsilon\eta_0\in\mathcal{O}$ for $\varepsilon\in[0,1)$; the same holds for $(-\eta_0)$. 
Hence, if $\mathfrak{P}(\eta(0))\ne 1$, the induction on $t\ge 0$ proves that
then $\mathfrak{P}(\eta(t))\ne 1$ for all $t$, and hence the opinions reach consensus.
%\end{proof}

\section*{Proof of Lemma~\ref{lem.n_3_no_period2}}

\textcolor{red}{TODO - proof in Appendix. Idea: assume without loss of generality that $d=2$ (we remain in 2-dimensional convex hull).
prove first the second statement: the area of the convex hull must be $0$ (unless this is an equilibrium). On the line, the minimal and maximal opinion also must remain unchanged - otherwise, they will never return to initial values. The remaining opinion should oscillate with period T. It remains to explain why $T>2$. I have the proof, but it's long.}


%\color{black}

%Здесь была тривиальная лемма, что кластеризованная матрица является равновесием тогда и только тогда, когда в каждой клике совдпадают мнения. Придется без нее.
\section*{Proof of Lemma~\ref{lem.clustered}}
If clustered opinion matrix $\Xi$ is an equilibrium of the GHK, then 
\[
\frac{1}{|\mathcal{N}_i(\Xi)|}\sum_{j\in\mathcal{N}_i(\Xi)}\xi^{j}=\xi^{k},\quad \forall i\in\V,k\in\mathcal{N}_i(\Xi),
\]
which entails the coincidence of opinions in each clique.

On the other hand, if for all $i,j\in\V$ either $\xi^i=\xi^j$ or $\xi^j-\xi^i\not\in\mathcal{O}$, then opinion matrix $\Xi$ is clustered and form an equilibrium because
\[
\frac{1}{|\mathcal{N}_i(\Xi)|}\sum_{j\in\mathcal{N}_i(\Xi)}\xi^{j}=\xi^{i},\quad \forall i\in\V.
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newpage

\appendix
\renewcommand{\theequation}{A.\arabic{equation}}
\setcounter{equation}{0}
%\section*{{$\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad$\it Appendix} } \label{sec:apCATD}


We will use a more compact representation of~\eqref{eq.HK}:
\begin{equation}
\Xi(t+1)=\Psi(\Xi)\dfb 
W(\Xi(t))\Xi(t),\;\;t=0,1,\ldots,\label{eq.Psi}
\end{equation}
where 
$W(t)\dfb W(\Xi(t))$ is the row-stochastic  
matrix whose entries (instantaneous influence weights) are defined as



\begin{comment}

\section*{Recurrent averaging inequalities}

%We will primarily deal with matrices that satisfy the following additional assumptions.
%\begin{assum}[\bf Type-symmetry]
%$\exists K \ge 1$ such that $w_{ij}(t) \le Kw_{ji}(t)$, %$\forall i,j \in [1:n]$, $t\ge 0$.
%\end{assum}
%\begin{assum}[\bf Type-symmetry]
%$w_{ii}(t) \ge \delta > 0$, $\forall i \in [1:n], t \ge 0$.
%\end{assum}


We primarily deal with matrices whose non-zero entries are \emph{uniformly positive}:
\begin{gather}\label{eq.uniformly_positive}
w_{ij}(t) \in \{0\} \cup [\delta, 1],\quad \forall i,j \in [1:n], t \ge 0,
\end{gather}
and diagonal entries are strictly separated from 0:
\begin{gather}\label{eq.uniformly_positive_diagonal}
w_{ii}(t)  \in [\delta, 1],\quad \forall i \in [1:n], t \ge 0.
\end{gather}


\begin{remark}\label{rem.matrices}
The Lemma~\ref{lm.consensus_alg} can be trivially extended to matrices $\Xi(t)\in\mathbb{R}^{n\times d}$ obeying the linear averaging dynamics 
\begin{gather}\label{eq.matrix-equation}
\Xi(t+1)= W(t)\Xi(t).
\end{gather}

Indeed, it suffices to apply Lemma~\ref{lm.consensus_alg} to columns $\xi_{*k}(t)=(\xi^1_k(t),\ldots,\xi^n_k(t))^{\top}$ of the matrix $\Xi(t)$ (that is, the vectors of the agents' opinions on topics $k=1,\ldots,d$).
\end{remark}


The following simple statement is proved via induction on $t=0,1,\ldots$
\begin{lemma}\label{lm.in_convex_set_forever}
Let $W(t)$ be a sequence of row-stochastic matrices, $G\subset\mathbb{R}^d$ be a convex set and the
sequence $\Xi(t)$ of matrices $n\times d$ be the solution of system~\eqref{eq.matrix-equation}.

If $G$ contains the rows $\xi^1(t_0),\ldots,\xi^n(t_0)$ of $\Xi(t_0)$, then it contains the rows of all subsequent matrices $\Xi(t)$, $\forall t\geq t_0$.\endofthm
\end{lemma}
\end{comment}

\section*{Proof of Theorem~\ref{thm.converg_HK}}

In this section, the assumptions of Theorem~\ref{thm.converg_HK} are supposed to hold.
Although formally Remark~\ref{rem.matrices} applies to \emph{linear} averaging  dynamics, it can be applied to particular solutions of the system~\eqref{eq.HK} by using the following standard trick.
\vspace{0.2cm}
\begin{lemma}\label{lm.rewritten_sys}
Let the confidence set satisfy Assumption~\ref{assum.Sym}. 
Consider a particular solution $\Xi(t)$ of  system~\eqref{eq.HK} and define $W(t)$ as in~\eqref{eq.W_GHK} (note that this matrix is determined by this specific solution). Then, $\Xi(t)$ is bounded, obeys~\eqref{eq.matrix-equation}, and $W(t)$ satisfies the conditions of Lemma~\ref{lm.consensus_alg}.
\end{lemma}
\begin{proof}
Obviously, matrices~\eqref{eq.W_GHK} are row-stochastic and $\Xi(t)$ is bounded equence in view of Lemma~\ref{lm.in_convex_set_forever}. Since $1\leq |\mathcal{N}_{i}(t)|\leq n$, one has
\[
\frac{1}{n}\le \frac{1}{|\mathcal{N}_{i}(t)|} \le 1.
\]
Using the latter inequality, one checks for all non-zero entries that
\[
w_{ij}(t) = \frac{1}{|\mathcal{N}_{i}(t)|} \ge \delta\dfb\frac{1}{n},
\]
and diagonal entries are strictly positive in view of Assumption~\ref{asm.0}.

%we obtain the diagonal elements are uniformly positive with $\delta = \frac{\varepsilon}{n}$.
Additionally, the sequence of matrices $W(t)$ is type-symmetric with $K\dfb n$.
\end{proof}

\begin{comment}
\subsubsection{\bf Proof of Theorem~\ref{thm.converg_HK}, statement (i)}

The first statement is straightforward from Lemma~\ref{lm.consensus_alg} (along with Remark~\ref{rem.matrices}) and Lemma~\ref{lm.rewritten_sys}.
Applying these lemmas to a particular solution of $\Xi(t)$, one proves the existence of the limits $\xi^i(\infty) =\lim_{t\rightarrow \infty}\xi^i(t)$, $i\in\V$. 

\subsubsection{\bf Proof of Theorem~\ref{thm.converg_HK}, statement (ii)}
If $\Xi = \Psi\Xi$, then $\Xi(t)\equiv\Xi$ is a solution to the SCOD system, and the corresponding matrix $W$ is constant $W(\Xi(t))\equiv W(\Xi)$.
Using Lemma~\ref{lm.consensus_alg}, $\xi^{i}=\xi^{j}$ whenever $w_{ij}\ne 0$, that is, $i\in\mathcal{N}_j$. This means that $\Xi$ is clustered: opinions of every two agents $i,j$ are coincident or ``dissimilar'' ($i\not\in\mathcal{N}_j$, $j\not\in\mathcal{N}_i$).

\subsubsection{\bf Proof of Theorem~\ref{thm.converg_HK}, other statements}

The proof of the remaining statements is divided into several steps. Henceforth we suppose that Assumption~\ref{assum.Zero} holds.

\textbf{Step 1. (Graph termination)} First we will show that confidence graphs $\mathcal{G}(t)$ converge in finite time.

%Since all non-zero entries $w_{ij}(t)$, thanks to~\eqref{eq.W_GHK}, are strictly positive:  $w_{ij}(t) = 1/|\mathcal{N}_{i}(t)| \geq \frac{1}{n}$, 
Lemma~\ref{lm.consensus_alg} entails the following implication:
If $\lim_{t\rightarrow \infty}\xi^i(t) \neq \lim_{t\rightarrow \infty}\xi^j(t)$ then $i \notin \mathcal{N}_{j}(t)$ for sufficiently large $t$. Indeed, if $i \in \mathcal{N}_{j}(t)$ for some sequence $t=t_k\to\infty$, then, trivially, $\sum_ {t = 0}^{\infty}w_{ij}(t) = \infty$ and hence the final opinion vectors $\xi^i,\xi^j$ must be coincident.

On the other hand, if $\lim_{t\rightarrow \infty}\xi^i(t) = \lim_{t\rightarrow \infty}\xi^j(t)$, then $i \in \mathcal{N}_{j}(t)$ for sufficiently large $t$. Indeed, in view of Assumption~\ref{assum.Zero}, there is $r > 0$ such that $B_{r}(0) \subset \mathcal{O}$. Since the limit opinions of agents $i$ and $j$ coincide then $\xi^i(t) - \xi^j(t) \in \mathcal{O}$ for sufficiently large $t$.

We have proved that, for each agent $i$, the set of ``trustees'' $\mathcal{N}_i(t)=\{j:\xi^j(\infty)=\xi^i(\infty)\}$ for $t$ being large. 
Hence, the graph stops changing at a certain time instant (depending on the solution). 
Moreover, agents belonging to the same cluster constitute a \emph{clique} in the terminal graph, and the nodes from different cliques are disconnected, that is $\Xi(\infty)$ is clustered.

\textbf{Step 2. (Opinions termination)} Since confidence graphs $\mathcal{G}(t)$ converge in finite time and the opinions of agents within each clique converge in one step to the average opinion, one arrives that convergence of opinions will occur no later than one step after the convergence of the confidence graphs. This proves (iii). 

In view of Lemma~\ref{lem.clustered} clustered opinion matrix $\Xi(\infty)$ form  form an equilibrium of the SCOD. This proves (iiii) and completes the proof of the theorem.

\end{comment}

\section*{Proof of Theorem~\ref{thm.converg_HK_stubborn}}
We will prove the theorem in the case $m=1$, that is, when there is one stubborn agent in the system with number $n+1$  ($m>1$ is proven similarly). Let us denote the set of ordinary agents by $\V'\dfb \V\setminus\{n+1\}$.
We will use the following lemma for future proof.
%\textcolor{red}{I would simplify the procedure and added $w_{i,n+1}$ to the diagonal instead of rescaling... On the other hand, rescaling can give some simplifications in the future analysis...}
\begin{lemma}\label{lm.subb}
The sequence $x_i(t) \dfb \|\xi^i(t) - \xi^{n+1}\|$ for $i\in\V'$ is bounded solution of~\eqref{eq.RAI} with $n\times n$ matrix $\widetilde{W}(t)$ defined as
%\begin{equation}\label{eq.W_GHK_stubb}
%\widetilde{w}_{ij}(t)\dfb \frac{w_{ij}(t)}{1-w_{i,n+1}(t)},\quad i,j\in\V',
%\end{equation}
where $w_{ij}(t)$ elements of the matrix $W(t)$ defined in~\eqref{eq.W_GHK}. Matrix $\widetilde{W}(t)$ satisfies the conditions of Lemma~\ref{lm.consensus_alg}.\endofthm
\end{lemma}
\begin{proof}
Obviously, matrices~\eqref{eq.W_GHK_stubb} are row-stochastic and the sequence $x_i(t)\ge0$ is bounded below.
Since 
\[
\|\xi^i(t+1)-\xi^{n+1}\| \le (1-w_{i,n+1}(t))\sum_{j=1}^n \widetilde{w}_{ij}(t)\|\xi^j(t)-\xi^{n+1}\|,
\]
one has
\[
x_i(t+1)\le (\widetilde{W}(t)x(t))_i.
\]


Since $0\le w_{i,n+1}(t)\le \frac{1}{2}$ for all $i\in\V'$ and $1\le|\mathcal{N}_i(t)|\le n+1$, one has
\[
\widetilde{w}_{ii}(t)\ge \delta \dfb \frac{1}{n+1}.
\]
Additionally, the sequence $\widetilde{W}(t)$ is type-symmetric with $K\dfb 2(n+1)$.
\end{proof}

\textbf{Proof of Theorem~\ref{thm.converg_HK_stubborn}.}
In view of Lemma~\ref{lm.subb}, Lemma~\ref{lm.consensus_alg} applies to the sequence $x_i(t) \dfb \|\xi^i(t) - \xi^{n+1}\|$ for $i\in\V'$, one proves the existence of the limits $x(\infty) \dfb\lim_{t\rightarrow \infty}x(t)$.


Note, that $x_i(\infty) = 0$ if and only if $\xi^i(\infty) = \xi^{n+1}$. Denote $I\dfb\{i\in\V':x_i(\infty) = 0\}$. Let's prove that agents from sets $I$ and $\V'\setminus I$ do not trust each other, for $t$ being large. 
Indeed, if for agents $i\in I$ and $j \in \V'\setminus I$ there is sequence $t=t_k\to\infty$ such that $w_{ij}(t)\ge\frac{1}{n+1}$ then, trivially, $\sum_ {t = 0}^{\infty}w_{ij}(t) = \infty$ and hence $\sum_ {t = 0}^{\infty}\widetilde{w}_{ij}(t) = \infty$, which implies $x_i(\infty)=x_j(\infty).$ 

As a result, the opinions of agents in set $I$ will converge to $\xi^{n+1}$, whereas the opinions of agents in $\V'\setminus I$ will behave as in a system without stubborn agent for $t$ being large and will converge according to the Theorem~\ref{thm.converg_HK}.

From statement (iii) of Lemma~\ref{lm.consensus_alg} we obtain that
\[
\Delta_i(t) = \sum_{j=1}^n \widetilde{w}_{ij}(t) x_j(t) - x_i(t+1) \rightarrow 0.
\]
Using the RAI estimate for the term $x_i(t+1)$ we obtain
\[
\Delta_i(t) \ge w_{i,n+1}(t){w}_{ii}(t) x_i(t) \ge 0.
\]
Since $\sum_ {t = 0}^{\infty}\widetilde{w}_{ii}(t)=\infty$, then $\sum_ {t = 0}^{\infty}w_{i,n+1}(t)=\infty$ implies $x_i(t)\rightarrow 0$ as $t\rightarrow\infty$. Thus, we have proven statement (ii) and thereby completed the proof of the theorem.

